The Excess Dissipation of Energy in a Turbulent Boundary-Layer and its Departure from Log-Normality

We investigate turbulent dissipation in a von Karman flow using PIV and Diffusing Wave Spectroscopy measurements to directly compare bulk and wall dynamics. While bulk dissipation conforms to the dissipative anomaly, wall dissipation exhibits a clear excess that grows with Re, consistent with velocity-gradient dominated scaling. Decomposition into dissipation intensity bands reveals that this excess is mainly driven by progressive redistribution toward high-intensity events, larger than 10 x mean, as Re increases. From these measurements, we infer the skin-friction coefficient, finding a decreasing trend with Re fairly consistent with classical power-law behavior despite increasing dissipation. Statistically, the wall shows strong departures from log-normality at low Re that diminishes with increasing Re, reflecting an increase in the effective dimensionality of the near-wall gradient field with Re. In contrast, the bulk dissipation remains near log-normal across all Re with slowly growing log-dissipation variance, consistent with K62 refined similarity. These results suggest distinct origins of log-normal behavior which are multiplicative cascade dynamics in the bulk versus the combined effect of persistent shear and a superposition of an increasing number of independent gradient contributions at the wall.

==> sections/discussion.tex <==


\begin{figure*}
\centerline{\includegraphics[scale=0.5]{figures/Eps_pdfs.png}}
\caption{\label{fig:PDFs} Probability density distributions of normalized dissipation, $\epsilon / \langle \epsilon \rangle $ (inserts), and centered-reduced dissipation, \logctrd, at two $Re$ for the DWS wall measurements and TPIV bulk measurements. The dashed black line shows a log-normal distribution, while in the inserts it shows a power-law fit to the left-tail, where the exponent is displayed in the text-box. 
%Note the distributions of the normalized and center-reduced dissipation signify different things, as they change which parts of the distribution dominate the physics. $\epsilon / \langle \epsilon \rangle $ is the most direct description of the flow field, and its moments are intrinsically sensitive to extremes. The distributions of \logctrd are more of a PDF shape or intermittency variable, as it turns multiplicative variation into additive, which ties into ideas that turbulent cascades are multiplicative. It isolates fluctuation relative to a local mean and compresses tails so that distributions are less dominated by extremes; making it more robust to shape comparisons across $Re$ or sample location.   
%Note biases: log compresses large values and amlifies small values 
 Low Re case looks very much like a Rayleigh distribution, which is a distribution of  a square of a variable with a normal distribution, indicating that velocity gradients are nearly gaussian. 
The fact that dist is clearly not symmetric and seemingly suppressed on the lower side. Data is not just non log-normal, but has directional structure in log space 
Rayleigh distribution means the variable behaves like the magnitude of a 2D latent Gausian process , in other words dissipation behaves more like a norm of a multicomponent random field than multiplicative cascade variable .
More structural intermittency - dissipation concentrated in localized strucutres 
Rayleigh instead of log-normal might also indicate low-dimensional dominant contributions , as in a few gradient components are dominating locally
}
\end{figure*}

\bigskip
\paragraph*{Results and Discussion}
\bigskip
\paragraph{Coherent Dissipation Structures} ~\\
We first note the structures seen in the dissipation fields shown in Figure \ref{fig:facility}c.
Here we see that dissipative action at the wall appears to occur within coherent structures with a preferred directionality and shape.
The structures are typically elongated along an axis that aligns most with the vertical axis of the facility - perpendicular to the azimuthal driving direction of the impellers. 
Further, as expected the size of these structures generally decreases with $Re$. 
The presence of coherent structures is notable as research by \citet{Dubrulle2019} highlighted the heightened importance of local dynamics and indicated that some of the highest energy transfer and dissipative events occur around coherent structures. 
Conversely, regions outside coherent resulted in behavior close to \citet{Kolmogorov1941}'s approximation with reduced intermittency.
\bigskip


\paragraph{Excess dissipation and $Re$ trend}~\\
Concerning dissipation statistics, we first consider the spatial-temporal average of the kinetic energy dissipation rate, \eps,  across all experimental runs performed at each $Re$. 
The extent of the spatial averaging is indicated in Figure \ref{fig:facility}a-c by the dotted blue line. 
The DWS \eps values measured at the wall are shown in Figure \ref{fig:mean_eps}a normalized by the theoretical dissipation rate for HIT flow: $\epsilon_{HIT} \propto U^3_{tip}/R$, where $U_{tip}$ is the velocity of the impeller tip at a given $Re$ \cite{Kolmogorov1941}. 
The dissipation rate measured by the facility's torque-meters, representing the global/volumetric dissipation of the flow, \epstrq, is also shown in Figure \ref{fig:mean_eps}a. 
Lastly, Figure \ref{fig:mean_eps}a includes the estimation of dissipation rate at the center of the von-Karman flow, \epsB, free of influence from boundaries and found previously to be in strong agreement with HIT estimates. 
These measurements were obtained using SPIV and TPIV diagnostics, and were taken in a range of previous works \cite{Debue2018,  Debue2021, Geneste2019, Musci2025}.
As observed in previous studies (\cite{Dubrulle2019, Dubrulle2022, Kuzzay2015,Saw2018}), when normalized the \epstrq and \epsB values approach a constant in bulk for $Re > 6000$; a manifestation of the 0th-law of turbulence, or the dissipative anomaly \cite{Iyer2025, Dubrulle2019, Drivas2018, Yao2020, Eyink2006}.  

Of the three dissipation measurements shown, \eps at the wall is always the largest, and thus in reference to the average global values, \epstrq , we have an ``excess" of dissipation at the wall. 
While it has been hypothesized that the high amounts of shear at the wall should locally increase the amount of turbulent kinetic energy production, which would in turn need to be dissipated by the flow, it is not at all obvious that this should occur locally at the wall. 
These measurements provide evidence that this is indeed the case. 

Furthermore, it is evident that \eps is increasing with $Re$.
In other words, the amount of excess dissipation is growing in the same flow where we experimentally observe 0-th law behavior in the volumetric and bulk measurements, \epstrq and \epsB. 
The contemporary DNS work of \citet{Duan2025} found similar results, albeit for wall generated turbulence where injected power through the boundary is likely $Re$ dependent. 
While observing near 0-th law behavior in the outer boundary layer region, they too found, friction Reynolds-dependent, excess dissipation at the wall which obeyed a ``bounded defect law."

% They observed 0th law behavior for dissipation in an outer region of turbulent boundary layer, while dissipation at the wall remained larger and grew with $Re_\tau$ (the friction $Re$) until some asymptotic limit, according to a ``bounded defect law."
% In our case, because we seek a normalization and $Re$ definition that is known apriori, and linked to the forcing/integral scale of the turbulent flow, we do not expect to recover such a law \cite{Duan2025}.
% However, we do see a qualitative agreement in that they observe an excess of dissipation at the wall which increases with $Re$, while dissipation in the outer-region remains more or less constant. 

%which found that for out-region wall bounded flows, when normalized the wall friction velocity dissipation for a first order moment, the avergare dissipation grows as $Re^{- 0.017}$ which could be interpreted as essentally a 0th-law result. %Similarly, they observe that wall dissipation remain larger than in the bulk, although with bounded growth when noralized byt the wall scale $\epsilon_\tau$. As we are instead normalizing by an apriori, outer inertial scale then the excess dissipation can grow with $Re$, providing qualitative aggreement with \citet{Duan2025}.
%However, even for a change of scaling, excess dissipation following a bounded defect law would still aproach an asymptitce value, which does not appear to be the case in our results as we fit an unbounded power law to our results. 

% For better comparison, we re-normalize the bounded defect law of \citet{Duan2025}. We assume that $Re_\tau \approx Re^{7/8}$, which is a common smooth-wall channel-flow approximation that is likely only valid here in an illustrative way. Re-normalizing \citet{Duan2025}'s bounded defect law by the relevant integral scale values, result in $\langle \epsilon \rangle / U_{tip}^3/R = (\alpha_p - \beta_p Re_\tau ^{-1/4}) \, Re_\tau^4 / Re^3$. The constants $\alpha_p$ and $\beta_p$ are on the order 0.1. 
% Thus, using the approximation for $Re_\tau$, to leading order mean dissipation normalized in our fashion would obey a bounded defect law if $\langle \epsilon \rangle / U_{tip}^3/R \propto Re^{1/2}$. 
% The amount by which normalized \eps increases with $Re$ is found via fit and shown in Figure \ref{fig:mean_eps}a. 
% While subject to several approximations and a relatively poor fit, we see a relation $\propto Re^{3/4}$, exceeding the bounded defect law criteria. 
% Nonetheless, even for a change of scaling and $Re$, a bounded defect law will by definition approach an asymptotic value, which does not seem to be the case here, at least for the range of $Re$ available in our study. 

Our results further add to the evidence of bulk turbulence obeying the dissipative anomaly, while simultaneously helping to clarify the previously observed dichotomy for a matching anomaly at the wall \cite{Eyink2024}.
It is noteworthy that we observe evidence for finite, and increasing, dissipation for increasing $Re$ at a smooth wall (although the flow is driven by ``rough" stirrers) as some works have observed decreasing dissipation for smooth walls, with others reporting 0th-law behavior for rough walls, wakes, and various boundary conditions \cite{Eyink2024}.
More importantly, unlike anomalous dissipation in the bulk, which has been clearly linked to limited regularity of the velocity field, walls introduce new mechanisms that can generate or suppress dissipation (via additional energy flux terms at the boundary) independent of any bulk mechanism. 
These findings highlights a gap in current turbulence theory, as the trends we observe are indicative of additional dissipation mechanisms that are not controlled by the regularity criteria which we simultaneously observe in the bulk.
%have found differnet dissipation beahvior at walls for differnt boundary conditions and wlal roughness. 
%Currently inssuficient evidence (numeric and experimental) to settle where a wall dissipation anamoly esits, or how it scales with $Re$
%Existing theory links anomalous dissipation in the bulk to limited regularity of weak solutions (Onsager framework), but provides no analogous closure for wall-bounded flows, where boundary layers introduce a

At minimum, these results seem to show that as $Re$ increases, boundary layer dissipation is increasingly decoupled from the integral-scale velocity $U$, or $\epsilon_{HIT}$. 
As such, we hypothesize that because velocity gradients at the wall must continually steepen with $Re$, wall dissipation becomes increasingly dominated by these gradients, and possibly by enhanced contributions from small scale shear at the boundary. 
That is to say, while we observe bulk flow dissipation to saturate with $\epsilon_{HIT}$ scaling (indicating HIT/cascade driven processes), wall dissipation is clearly velocity-gradient driven and increases at a faster rate than bulk dissipation. 

%As such, if we assume to leading order that at the wall, $\epsilon \approx \nu (\frac{\partial u}{\partial y})^2$, then how the velocity gradient grows with $Re$ determines how \eps scales with $Re$.
As such, we take a dimensional-analysis perspective and assume:
\begin{equation}
 \epsilon_{wall} \approx u_\tau ^4 / \nu  \; ,
 \label{eq:eps_dim}
\end{equation}

\noindent where $u_\tau = \sqrt{\tau_\omega / \rho}$ is the friction velocity (and $\tau_\omega$ the wall shear-stress). 
One can then link $u_\tau$ and $U$ via the skin friction coefficient, $C_f = 8 \tau_\omega / \rho U^2 $. 
For illustrative purposes, we know from classical flat-plate and pipe flow experiments that the skin friction is weakly dependent on $Re$, such that $C_f \propto Re^{-n}$, where usually $n < 0.25$ \cite{White2006, Schlichting2016}. 
With these relations we can then estimate, to leading order, how dissipation at the wall might scale with the integral $Re$ via $\epsilon_{wall} \approx U^3 Re^{1-2n} / R$.
That is, as long as $n < 0.5$, we should expect $ \epsilon_{wall} / \epsilon_{HIT}$ to grow with $Re$, as observed in Figure \ref{fig:mean_eps}a.

This line of reasoning can then be used to show that DWS allows for the experimental measurement of $C_f$. 
Again starting from the assumption of Equation \ref{eq:eps_dim}, and using the relations introduced above, one can see that $C_f \approx 8\sqrt{ \langle \epsilon \rangle R \, / \, U^3 Re}$.
Figure \ref{fig:mean_eps}b shows that this decreasing trend is observed for the experimental $C_f$ values.
The various lines shown in Figure \ref{fig:mean_eps}b are for different flow forcings, where Anti and Con indicate curved impellers rotating in the scooping and non-scooping directions, respectively, while Frac indicates straight blade impellers machined in a self-similar/fractal pattern. 

As empirical relations for $C_f$ do not exist for the von Karman flow, we again use axial pressure-gradient pipe flow measurements for an illustrative comparison.
The seminal work of \citet{McKeon2005} empirically established that $C_f$ varies with $Re$ according to Prandtl's log-law theory \cite{Prandtl1905, McKeon2005, Dubrulle2024}. 
However, as established in \citet{Dubrulle2024}, in the low-mid $Re$ range, the log-law theory is nearly indecipherable from the Blasius power-law relation of $C_f = 0.3164\, Re^{-1/4}$ which we use here \cite{Blasius1913,  McKeon2005}. 
The power-law fits to the data in Figure \ref{fig:mean_eps}b show $C_f$ behavior within reasonable agreement of this trend. 

The different absolute values of $C_f$ for each of the forcings at a given $Re$ could be equated to an effective boundary roughness caused by the impellers. 
Although the cylindrical-wall boundary of the facility is very smooth, the effective roughness felt by the flow appears to change depending on the impeller used. This is apparently tied to the degree of turbulent fluctuations induced by an impeller type.
For instance, previous works have found Anti to produce higher turbulent intensities as compared to Con for the same integral scale $Re$ \cite{Ravelet2004, Saint-Michel2013,Dubrulle2022} 
This can be inked to the Taylor Reynolds number, $Re_\lambda$, in that while a given integral $Re$ can be equivalent for different impeller types, because each impeller has been found to cause different amounts of volumetric dissipation and turbulent intensity, each must then have a different Kolmogorov and Taylor length scale for a given $Re$. 
Thus, $C_f$ seems to be linked more intimately with turbulent fluctuations than with integral scale forcing. 

More generally, the observation that $C_f$ decreases with $Re$, while dissipation increases is a non-trivial point.
This indicates that velocity gradients are being amplified enough by turbulence to increase dissipation, despite a simultaneous weakening of the wall stress relative to $U^2$.
The general agreement with the traditional skin friction behavior adds to the appeal of the DWS technique, as it offers an avenue for directly estimating $C_f$. 

These results add subtle context to the pioneering work of \citet{Cadot1997}, which found that boundary layer dissipation controlled global dissipation scaling as a drag coefficient decreased.
Our findings show that this behavior arises because wall dissipation is controlled by velocity gradients tied to skin friction, not by $U$, leading to the breakdown of global normalization.  
However, their argument that a decreasing $C_f$ at the boundary will lead to dissipation and drag dominated by the bulk, seems to be in conflict with our finding that one can have \eps excess increase at the wall in conjunction with a decreasing $C_f$.

\begin{figure}
\centerline{\includegraphics[scale=0.4]{figures/StatMoms_vs_Re.png}}
\caption{\label{fig:stat_moms} 2nd-4th order statistical moments of $\chi = \ln ( \epsilon / \langle \epsilon \rangle )$ for wall DWS (blue circles) and bulk PIV (gold triangles) measurements.  }
\end{figure}



\bigskip
\paragraph{Distributions of $\epsilon$}~\\
For further insights into the dissipation at the wall we turn to it's distributions and higher-order moments.
We show the normalized ($\, \epsilon /$\eps  $\,$) and center-reduced ($\,$\logctrd $\,$) dissipation distributions for the wall and flow bulk for low and high $Re$ in Figure \ref{fig:PDFs}.
We first note that the normalized distributions (inserts), show greatly varying left tail characteristics for the wall and bulk measurements. 
Generally, at the wall the left tail slope is near 0, indicating a large influence of near-zero dissipation events. Further, a negative slope would indicate a divergent PDF for zero dissipation. 
As $Re$ increases (Figure \ref{fig:PDFs}b) we see the slope grow and the dominance of near-zero events decrease. 
Conversely, near the flow center the steeply positive left tail slopes indicate a vanishing PDF for zero dissipation events, meaning the bulk is more strongly protected against near-zero dissipation.
These differences may hint at varying mechanisms of energy cascade and intermittency for the wall versus the bulk, where the high shear rates experienced at the wall may somehow serve to enhance the probability of low-dissipation events in comparison to the bulk.  

Previous works have found similar results for the bulk, arguing that HIT flow should have a left tail power-law exponent near 1.5 \cite{Duan2025, Gotoh2023, Elsinga2023}.
Departure from this value is argued to be due to the relative number of velocity-gradient terms (e.g. $\epsilon_{uu} = \nu \partial_ju \partial_j u $) actively contributing to dissipation. 
With this interpretation, a left-tail slope near 0 corresponds to two velocity gradient terms contributing to the dissipation at the wall, whereas a slope of 2 for the bulk indicates contribution from 6 terms \cite{Gotoh2023}.
This would suggest that wall/bulk left-tail difference should be read first as a difference in the kinematic structure of the dissipation observable, not immediately as stronger/weaker multi-fractality \cite{Ruiz-chavarria2000}.
That is, as $\epsilon$ is essentially a sum of squared velocity gradients, $\epsilon \approx 0$ requires all the summed gradients to be negligible. 
This would be increasingly improbable the more active velocity gradients there are. 
Thus, any non-zero dissipation at the wall is likely built from only a few independent velocity gradients, allowing for both the diverging left tail and the large mean \eps seen in Figure \ref{fig:mean_eps}a. 

% \cite{Ruiz-chavarria2000}: show dissip stats are shaped by kinematic contraints and dyanmical organiztion. Shows that higher order velo stats are governed by intense and lcoaclized eents. Found that shear-driven dissiaption became increasinly intense with Re. shows mechanis for a higher \eps at wall due to persistent high shear ath the wall, with a more intemrittent bulk that has intense shear vents more spatailly intermittent  - the bulk increase intemrritceny through raree, but more extreme events compared to the wall.
% They also find pdf and struture uncs of vel incermemtns depends strongly onwall distance, and that also they depend on resolution/scale in the loglayer, where smaller scales show more HIT-like behaviour. 
% Tehy show shear dominated sclaing near wall 


Concerning the center-reduced distributions in the main panels of Figure \ref{fig:PDFs}, one can see that the bulk PDFs remain quite close to log-normal (dotted-line) for both $Re$ cases, as predicted by \citet{Kolmogorov1962} (hereafter K62). 
On the other hand, the distribution at the wall displays a strong asymmetry at low $Re$ (Figure \ref{fig:PDFs}a), with a strong left-tail and relatively weak right tail; a distinct departure from log-normality.
In fact, the PDF is more closely aligned with a Chi-squared distribution ($\chi_k^2$) with $k=2$, otherwise known as a Rayleigh distribution (dashed-line). 
The right tail is particularity well captured by this distribution, which may mean high-dissipation events behave like the squared magnitude of a two component velocity gradient vector, which itself has a Gaussian distribution.  
This aligns directly with the normalized PDF left-tail interpretations of  \citet{Gotoh2023} and \citet{Ruiz-chavarria2000} discussed above: dissipation bursts are controlled by a small number (i.e. 2) of dominant velocity gradient components.
However, the faster decay of the low dissipation events and the higher/narrower peak (misleadingly suppressed in a log-y scale but very apparent in a linear scale, although not shown) as compared to Rayleigh indicate this is not a wholly adequate model.
Instead, our data seems to have a dissipation floor that is more constrained by a persistent background dissipation level. 
This could in turn be interpreted as a sustained background shear, or organized boundary layer, state on which fluctuations are superimposed. 

In Figure \ref{fig:PDFs}b's case of higher $Re$, these features are softened but generally still present. 
The left tail still appears stronger than the right, although the positive dissipation extremes are now closer to log-normal. 
We also see that for this $Re$ both tails of the wall dissipation are captured more closely by a $\chi_k^2$-distribution, albeit with $k \approx 30$.
We should not interpret this to mean that 30 gradient terms are now contributing to dissipation, as resolution, coarse-graining, averaging, etc.\ could be at play at the higher $Re$.
However, one can confidently say the number of degrees of freedom in the wall dissipation has increased, where \eps is now a more composite quantity at higher $Re$.
This could be due to an increase of independent squared velocity gradient contributions now contributing to dissipation, the development of more small-scale structures than at lower $Re$, or increased cascade-like multiplicativity.
In addition, the data distribution's peak is more in line with the log-normal and $\chi_k^2$-distributions, signifying the erosion of a preferred/organized dissipation level.
Finally, while the degree of asymmetry has clearly lessened, it is still more pronounced as compared to the bulk flow. 
%BUT often the better variable for comparing relative fluctuation structure, but worse for judging the absolute burden of intense dissipation events . NOTE if two datasets have similar cHi-distributions but different mean eps, then they have similar relative intermittency but not similar absolute dissipation. If two datasets have similar eps/mean(eps) tails but different chi skewness/kurtosis, then the tail energetics may match while the bulk/log-shape does not. 


\bigskip
\paragraph{Higher-order statistical moments of $\epsilon$}~\\
To better interpret the different trends of mean dissipation displayed in Figure \ref{fig:mean_eps}, we examine the next three statistical moments: variance, skewness and kurtosis. 
These results are shown for the log-normalized statistics, $\chi$, in Figure \ref{fig:stat_moms}. 
Here $\chi = \ln ( \,\epsilon / \langle \epsilon \rangle\, )$ for the respective dissipation measurements at the wall and bulk.   
One can see that at the wall, there are fairly clear trends of decreasing variance, increasing skewness and decreasing kurtosis with $Re$. 
Conversely, in the flow bulk we see variance increasing, although to a lesser degree, while kurtosis and skewness are approximately constant with $Re$. 
Thus the excess dissipation effect manifests markedly in the higher order moments of $\chi$ at the wall as compared to the bulk.

%Thus in the bulk flow we observe a broadening of the distribution, strengthening right tail, and larger influence of extreme dissipation events; indicating that intermittency is strengthening with $Re$ in the classical sense.
In terms of the bulk flow $\chi$ moments, the variance close to 1, skewness of 0 and kurtosis of 3 indicate distributions quite close to log-normal, aligning with the refined hypothesis of K62, re-affirming that we see HIT dissipation behavior in the bulk. 
This reinforces the classical picture of turbulence at the flow center, where intermittency increases with $Re$ and dissipation is driven by the cascade mechanism.

At the wall, the higher order $\chi$ moments show a different picture. 
Concerning variance, the decreasing trend with $Re$ signifies that the spread of fluctuations in log space is shrinking, or the relative fluctuations in dissipation are decreasing, indicating that dissipation is more tightly distributed around its mean as large excursion are increasingly compressed.
For skewness, the initially negative values represent a strong left tail, corresponding to high numbers of very weak dissipative events. 
% In other words, at low $Re$ there are frequent low-dissipative states with rare spikes up. 
As $Re$ increases, the left tail weakens and the distribution becomes more symmetric, with the very weak dissipative events becoming less dominant.
With kurtosis, at low $Re$ we see a highly intermittent and heavily tailed distribution signifying more extreme, infrequent events as opposed to frequent smaller deviations from the mean.
As $Re$ increases, we observe a decrease in intermittency via the gradual loss of heavy tails and extreme events. 

5
% Quantifying intermittency can also be done by looking at arbitrarily higher order normalized moments, $I_P = \langle \epsilon^p \rangle / \langle \epsilon \rangle ^p$, which are shown in Figure \ref{fig:Ip}.
% Here we see that, for a given $Re$, the growth of $I_p$ in the flow bulk far outpaces that at the wall, which is in agreement with the findings of \citet{Duan2025} who found that their bulk flow had a p-dependent intermittency correction which increases with $Re$, whereas the wall's remained bounded. 
% This provides further evidence that intermittency plays a stronger effect in the flow bulk than at the wall.
% If the bulk has larger $I_p$ than at the wall, it is consistent with the bulk containing stronger mean-normalized high-transfer/high-dissipation events, even if the wall has more distorted $\chi$ PDFs (Figure \ref{fig:PDFs}).

\bigskip
\bigskip
\paragraph{Interpretation of excess dissipation}
 : \\\\ 
  \begin{figure}
\centerline{\includegraphics[scale=0.58]{figures/Cont_bands.png}}
\caption{\label{fig:ContBnds} Contribution of banded events to the mean \eps shown in Figure \ref{fig:mean_eps} for the bulk (hatched bars) and the wall (solid color bars). The bulk bands undergo much smaller changes across the probed $Re$ range and are thus only shown at the two edges of their range. $C_{a-b} = \sum_{a < z_i < b} \epsilon_i / \sum_i \epsilon_i$, where $z_i = \epsilon_i / \langle \epsilon \rangle$. Figure \ref{fig:ContBnds} shows that the contribution ot mean dissipation at in the bulk is roughly invariant, with marginal increases in events $> 2$ \eps resulting in a minor decrease in contribution from all events $< 2$ \eps. On the other hand the wall shows a clearer redistribution toward the higher bands as $Re$ increases. At low $Re$ the events $< 2$\eps are the major contribution to \eps, with events 2-5\eps being close behind (combined $\approx 85 \%$). The contribution of these bands both shrink as $Re$ increases (combined $\approx 70\%$) and are displaced primarily by the contribution of extreme events ( $ > 10$\eps). $C_{10-50}$ in particular increase from a 2$\%$ to a $13\%$ contribution to the mean dissipation. Thus more of the dissipation is coming from increasingly intense events, which could be interpreted as increased intermittency as localized high dissipation events contribute more disproportionally to \eps at the wall. 
}
\end{figure}

Overall, the $\chi$ moment trends at the wall display a change from highly 
non-log-normal distributions toward more Gaussian ones at higher $Re$. A 
naive reading might interpret this as decreasing wall intermittency with $Re$. 
However, intermittency is properly defined through deviations of velocity 
increments from Gaussianity, not through dissipation PDF shape, and our 
band decomposition in Figure~\ref{fig:ContBnds} provides a concrete reason 
to resist this interpretation. The bulk band contributions are largely 
invariant across the probed $Re$ range, reflecting the self-similar cascade 
statistics already evidenced by the near-constant $\chi$ moments in the bulk. 
The wall, by contrast, undergoes a clear redistribution: at low $Re$, wall 
dissipation is dominated by events $< 2\langle\epsilon\rangle$ and 
$2$-$5\langle\epsilon\rangle$ (combined $\approx 85\%$). As $Re$ increases, 
these low-intensity contributions shrink to $\approx 70\%$, displaced by 
extreme events $> 10\langle\epsilon\rangle$, with $C_{10\text{-}50}$ alone 
growing from $2\%$ to $13\%$ of the mean dissipation. This redistribution 
is the direct cause of the rising normalized wall mean, and reflects that 
high-dissipation events are contributing increasingly disproportionately to 
$\langle\epsilon\rangle$ at the wall. That the distribution simultaneously 
becomes more log-normal is not in conflict with this: at low $Re$ the wall 
right tail decays faster than log-normal, so the transition toward log-normal 
statistics necessarily entails a heavier right tail and more extreme events. 
The apparent tension between increasing log-normality and increasing 
extreme-event contributions is precisely what demonstrates that PDF departure 
from log-normality is a poor proxy for intermittency. At the wall, the two 
evolve in opposite directions with $Re$.

Rather than reflecting intermittency in the classical sense, the decreasing 
departure from log-normality is more plausibly explained by an increase in 
the effective dimensionality of the near-wall gradient field, as evidenced 
by the transition from $\chi^2(k=2)$ to $\chi^2(k=30)$ statistics with $Re$. 
At low $Re$, only a small number of independent gradient contributions 
dominate the dissipation field, producing the strongly asymmetric, 
low-dimensional statistics observed. As $Re$ increases, more structures 
contribute to the near-wall velocity gradient — consistent with the 
$C_f$ trends and the findings of \citet{McKeon2005, Dubrulle2024}, who 
emphasize that skin friction increasingly depends on the specific velocity 
profile structure as $Re$ increases. When many such contributions combine, 
an effective multiplicative stochastic process emerges, driving the 
distribution toward log-normality regardless of whether a cascade mechanism 
is present. Thus, wall log-normality at high $Re$ reflects structural 
superposition at the boundary rather than any mechanism specific to the 
inertial cascade.

The relationship between PDF shape and intermittency at the wall is therefore 
not straightforward, and our results caution against conflating the two. 
Work by \citet{Elsinga2023} suggests that higher-order moments are primarily 
controlled by large-scale shear layers, with the left tail being most 
non-log-normal. At the wall, however, shear layers are a permanent boundary 
condition rather than an intermittent mechanism — persistent and space-filling 
rather than sparse and intense. This could explain how the wall simultaneously 
sustains a strongly distorted dissipation PDF and elevated mean dissipation, 
while the departure from log-normality reflects persistent shear-driven 
spatial organization rather than intermittency in the cascade sense. This 
interpretation is consistent with the findings of \citet{Duan2025}, who 
showed the wall region to be increasingly non-intermittent, and with the 
emphasis of \citet{Dubrulle2019} on local inertial energy transfer as the 
more appropriate lens through which to understand intermittency corrections. 
Near the wall, persistent geometry-imposed shear strongly reshapes the 
dissipation field and breaks local universality, yet does not automatically 
produce stronger high-order intermittency.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Intermittency is measured by deviation of velocity  from Gaussianity , not log-normality!

% Overall, the $\chi$ moments trends at the wall display a change from highly non-lognormal distributions, to those that are more gaussian at higher $Re$. 
% If one interprets higher departure from log-normality as higher intermittency, than this suggests that near the boundary intermittency is decreasing with $Re$, opposite of what is generally though to occur in the bulk. 
% %Perhaps this could indicate boundary layer dissipation that transitions from a regime dominated by bursts and intermittency/rare-events to one where many independent contributions cancel out to create more gaussian/log-normal like behavior. 
% The increasing log-normality could be associated with an increasing number of degrees of freedom at the wall (due to increasing eddy interactions, for example), an increased degree of mixing (with dissipation becoming less localized via the enhanced creation of small scale structures), or just the reduced dominance of rare events. 
% Alternatively, since we expect spatially inhomogeneous flow at boundaries, perhaps the departure from log-normality at lower $Re$ is the manifestations of dissipation occurring in localized structures (shear layers, hairpin vortices breakdown, etc.).

% Crucially, when we couple these findings with the mean dissipation trends discussed above (Figure \ref{fig:mean_eps}a), we can see that at lower $Re$ wall dissipation is more dominated by bursts and high intermittency, whereas at higher $Re$ we observe a more gaussian but continuously active dissipation field (hence the higher mean) - i.e dissipation is persistently high everywhere near the wall. 
% However, it also indicates that we are seeing log-normal stats emerge from two physically different mechanisms: multiplicative energy cascade in the bulk (K62 multiplicative energy transfer across scales) vs velocity gradient dominated flow at the wall. 
% Yet, log normality can arise generally when a mechanism is the product of many weakly dependent positive factors, which would only be possible at the wall if the dominant velocity gradient was not a single scale object and was instead influenced by things such as outer-layer large scales, wall attached eddies, hairpin vortices, near-wall streaks, or viscous sublayer dynamics. 
% When contributing together, these features might then lead to an effective multiplicative stochastic process represented by a log-normal distribution.
% That is, despite fundamentally different physical mechanisms governing dissipation in the bulk (cascade-driven) and at the boundary (gradient-driven), both regimes converge toward log-normal statistics at high $Re$. 
% This would suggest that wall log-normality reflects an underlying multiplicative stochastic structure rather than a mechanism specific to the inertial cascade.

% The idea that an increasing amount of contributing structures could push towards more log-normal statistics is also supported by the observed trends in $C_f$. 
% Findings in \citet{McKeon2005, Dubrulle2024} emphasize that the skin friction, and thereby dissipation, increasingly depends on the specific velocity profile structure at the wall as $Re$ increases. 
% Thus, wall shear remains dynamically important and more structures likely contribute to the near-wall velocity gradient  as $Re$ increases.
% %This could be why we observe higher mean dissipation yet reduced intermittency relative to the bulk. 
% %This suggests that log-normality may extend beyond the intertial cascade and is in line with refined simialryi adn mutifractal interprestaions of turbulence. 
% %As $Re$ increases we see the distribution becoming more symmetric and becoming less dominated by extremely small eps/mena(eps) values. higher Re  may be producing a more organized or less under-dissipative normalized background, while still generating more powerful intense dissipation bursts


% % SKEW is asymetrry, posotive skew is right tail longer and mean is usually greater than median, bulk of data on left. ------- 
% % -------For Trends in epsilon, increaseing higher order moemtns with Re signifies that in linear space dissipation field is becoming more intermittent, right tail is becoming more influential, burts matter more as they contribute with increasing strenght to higher order stats. 
% % ------ Trends in Chi say that dist is not getting broader, but its core is tightening, and its tails are becoming less heavy on both sides, while dist is becoming more asymettric . 
% % So as Re increase nomralized didspation is developing a tighter background in log space, with intense dissip events becoming more one sided and more effective at populating the right tail - these asymetric extremes dominate the raw eps moments.  ----


% %  \begin{figure}
% % \centerline{\includegraphics[scale=0.4]{figures/Ip_exp.PNG}}
% % \caption{\label{fig:Ip} PLACEHOLDER P-th order normalized statistical moments $(I_p = \langle \epsilon^p \rangle / \langle \epsilon \rangle ^p )$ at one $Re$ for the DWS wall measurements and TPIV center measurements. The faster growth of $I_p$ in the bulk indicates stronger intermittency as compared to the wall. 
% % %X-axis is p, y-axis is $I_p$.  As faster $I_p$ growth indicates stronger intermittency, we see that the the bulk is more intermittent, such that rare intense dissipation events contribute more strongly to the mean. Although the wall-region center-reduced PDF departs more strongly from lognormal, here the bulk exhibits larger normalized dissipation moments $I_p$. This indicates that non-log-normality near the wall is not synonymous with stronger high-order intermittency; rather, the wall departure appears to reflect wall-induced asymmetry/inhomogeneity, whereas the bulk has the stronger mean-normalized contribution from intense dissipation events.
% % }
% % \end{figure}




% These observations could have particular importance as previous research by \citet{Dubrulle2019} has highlighted the heightened importance of local dynamics in the highly inhomogeneous nature of scale to scale energy transfer and viscous dissipation, while regions of low local inertial energy transfer resulted in reduced intermittency.  
% Higher $I_p$ in the bulk than at the wall would seem to support this idea that intermittency is tied more to strong local energy-transfer events rather than to PDF non-log-normality alone.
% Several works have indicated that some of the highest inter-scale energy transfer events occur around coherent structures, indicating that the wall/bulk difference observed here is probably not just ``more or less intermittency” but a difference in how dissipation is spatially organized and which structures dominate it.
% Thus, the clear presence of coherent structures in the wall dissipation fields (Figure \ref{fig:facility}c-d) may explain the move towards the log-normal characteristics of $\chi$ seen in Figure \ref{fig:stat_moms}, while still observing larger $I_p$ moments in the bulk. 
% That is, at the wall, departures from log-normal seem to be decoupled from intermittency increases. 


% Again considering the results of Figure \ref{fig:mean_eps}a, if the wall has higher \eps but  shows a weaker $I_p$ trend as compared to the bulk, then one plausible reading is that the wall sustains stronger mean dissipation thanks to persistent shear-driven structures. 
% Conversely, the bulk sustains higher intermittency because of more cascade-dominated extreme events.
% This is a concrete piece of evidence that “departure from log normality” and “strength of intermittency” are not interchangeable; that intermittency corrections may be better understood through local inertial energy transfer approaches (à la \citet{Dubrulle2019}) than through coarse grained, ensemble, dissipation moments.


% Another interpretation as to why the wall can show larger PDF distortion and higher mean dissipation, but relatively smaller $I_p$ (intermittency growth) than the bulk can be found in \citet{Elsinga2023}. 
% This work further supports the idea of separating PDF shape from $I_p$ growth, as they show higher-order moments and intermittency to be primarily controlled by large-scale shear layers and the contributions they make to the distribution tails. 
% They note in particular that the left tail/low dissipation side of the PDF is most non-lognormal. 
% If this is indeed the case, the bulk is made intermittent by intense shear layers which are sparse intense events sitting in a quieter dissipation background.
% However, at the wall, this cannot be the case, as wall-shear layers are a permanent boundary condition rather than an intermittent mechanism. 
% This is also supported by the findings of \citet{Duan2025}, who showed the wall region to be increasingly non-intermittent.
% As such, the wall shear layers can provide larger PDF distortion and mean dissipation, while remaining less intermittent/lower $I_p$ than the bulk. 
% Thus near the wall, the shear is persistent, imposed by geometry and space-filling such that it strongly reshapes the dissipation field, breaks HIT/local universality, and changes the PDF shape, yet that does not automatically produce larger high-order intermittency

% %- \citet{Elsinga2023} argues dissipation intermittency is shaped most by large-scale shear layers, and the development of these layers cause $Re$ dependent scaling of dissipation moments and extremes.
% %explicitly say the low-magnitude tail is governed by a different framework: a Gaussian-random-field argument tied to the number of velocity-gradient terms, not by the lognormal/shear-layer model they use for the high tail.. 
% %These findings indicate that greater departure from log-normality at the wall is not equivalent to greater intermittency in the sense of Reynolds-number growth of high-order moments.

% % \cite{Duan2025} Intermittency of energy dissipation has long been studied via high-order moments in homogeneous and isotropic turbulence (HIT) in HIT, energy cascades from L to eta. In inertial HIT, inertial rang ei selfsimilar and inviscid, this leds to unveirsal structure funciton realtiron for turb. this is broken by intermittency, as structure functions differ for each moment.
% % near wall strong mean sher breaks HIT, and small scale features are directly impacted by large scale features (wall) - so they are not locally universal. in theory vel must rech 0 at the wall, while dissipation should reach a maximum
% % - showed disipation to have a some preferential direction/oriantaion as compared to the center
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bigskip
\bigskip
\bigskip
\bigskip
\paragraph{Boundary Layer considerations}
 : \\\\
% -DISCUSS HOW WHAT WE KNOW ABOUT THE BOUNDARY LAYER MIGHT BE INFLUENCING OUR MEASUREMENTS OR CAUSING THE EXCESS
\bigskip
\bigskip
\bigskip
\bigskip

\paragraph{Conclusions}
 : \\\\
 These results show that near-wall dissipation remains finite and even increases with Reynolds number while likely becoming less intermittent.
 This indicates that dissipation could be generated by distributed boundary-layer gradients rather than bulk singularities.
 In general it highlights a fundamental gap in turbulence theory, since existing frameworks (Onsager/Kato) do not provide a predictive description of how wall-bounded dissipation scales or organizes statistically \cite{Eyink2024}.
 Further, assuming the validity of Equation \ref{eq:eps_dim}, these results point towards a unified framework of wall turbulence that must simultaneously achieve $C_f \approx Re^{-n}, \; \epsilon \approx Re^{1-2n}$, while possibly decreasing intermittency.
 These observations provide evidence for the development of a unified framework connecting skin friction laws, dissipative scaling, and intermittency in wall-bounded flows.
 Finally, they support the idea that intermittency and log-normality in turbulent boundary layers are not strongly coupled, and that intermittency corrections may be better understood through coherent structures and local-dynamics. 
 The dissipation PDFs at low Reynolds number are consistent with Rayleigh or low-degree chi-square statistics, indicating that wall dissipation is governed by a small number of dominant gradient components. At higher Reynolds number, the distributions shift toward higher-degree chi-square–like behavior, suggesting that dissipation arises from a superposition of many contributions, either due to increased turbulence complexity or spatial coarse-graining. This transition reflects a change from shear-dominated to more distributed dissipation dynamics at the wall.
 \bigskip
\bigskip
\bigskip
\bigskip
% \citet{Duan2025} found that dissiaption matched a bounded defect wall and exhbited a non-intermittent character of dissipative vents, while also pbserving the mean to be larger than the bulk.
% supports idea that there is a limit to the grid resoltuion needed for resolving dissipation at the wall, due to this lack of intermittency there.
% - note that gammaP is the correction of K41 to intermittency, if gammaPis 0 we have k41, they find gmampP to be less than 0, whihc htye interpret as vanishingly small dissip in the bulk,compared to that on the wall, for very large Reynolds
% numbers. This means that away from the wall, the flow
% does not generate sufficiently strong singularities. However, the extreme nature of dissipative events on the wall
% (compared to those in the bulk of the channel) suggests
% that walls may generate the necessary strength of singularities. This brings us to the broader possibility that
% the Onsager-type singularities [48, 49] might be generated only near the wall. (THIS SEEM CONTRADICTORY TO THE FACT THE WE ARE LOSING INTERMITTENCY AT THE WALL)

% Overall, if $\chi$ at the wall was well described by a simple gaussian distribution whose variance alone changed with $Re$, then dissipative behavior would be tied mostly to variance, which is the classical refined-similarity picture of K62. 
% For modeling implications, the fact that the raw moments of \eps increase, while the variance of $\chi$ decrease with $Re$, indicates that a one-parameter lognormal interpretation is too simplified for dissipation at the wall. In general, the deviation from log-normality indicates a cascade mechanism at the wall which trasfers and dissipates energy differently than that of HIT flows.


% Not “everything is spreading out,” but rather “the bulk tightens while the high-dissipation side becomes more structurally distinct.” That is also a sign that a simple lognormal model is probably insufficient. If Chi were truly close to Gaussian across Re then its skewness would stay near zero and the increase of eps moments would be tied mainly to increasing var(chi). Your observation that Var(chi) decreases while raw eps moments increase says the Reynolds-number evolution is being carried by non-Gaussian structure in Chi especially asymmetry, rather than by a single widening lognormal parameter. 
% ---- NOTE for skewness, Chi is going from very negaitve ot less negative, close to 0, that indciats it originally has a pronounced left tail correpsonding to many very weak events, so as it approaches 0 it is acutally becomeing more symetric, and narrower: Increasing RE does not appear to make the log-dissipation field uniformly broader. Instead, it makes the chi-distribution less dominated by very low dissipation, while the intense positive dissipation events become more important in linear space and therefore drive up the raw eps variance, skewness, and kurtosis 







% BL SOURCES:
% - Lund (1994) LES demonstrate that concave curvature leads to significant changes in boundary-layer statistics, including increased skin friction, altered mean velocity profiles, and enhanced Reynolds shear stress, particularly through the action of curvature-induced secondary motions such as Taylor–Görtler vortices. These vortices generate alternating regions of upwash and downwash that transport high-momentum fluid toward and away from the wall, thereby increasing near-wall shear and modifying the distribution of turbulence production and dissipation.  curvature effects directly influence the near-wall region-  the resulting turbulence is strongly non-equilibrium, with local statistics departing from those of flat-plate boundary layers. 

% - Patel (1969) demonstrates that even moderate curvature produces substantial departures from flat-surface behavior, affecting velocity profiles, shape factor evolution, entrainment, and the overall growth of the boundary layer. A central finding is that the conventional flat-surface momentum integral equation fails when there are significant static-pressure variations across the boundary layer, which arise naturally due to streamline curvature, and that these pressure-gradient terms can be comparable to or larger than skin-friction contributions. 
% paper derives a modified momentum integral equation for boundary layers on surfaces of constant curvature, which explicitly includes curvature-induced pressure terms and provides improved agreement with experimental measurements. 
% establishes that curvature introduces first-order effects on turbulent boundary-layer dynamics and energetics, and that accurate descriptions of wall-bounded turbulent flows on curved surfaces require explicit consideration of streamline curvature

% -on concave suraces Gortler instbaility can cause a destabilization of BL which increase mixing and skin friction and substantially increases the BL thickness . Gorlter number  used to see whether it is causes intasbility, G higher than 0.3 means have gotler instbaility vortices , our qunifity as BL-thicknes/R and anything larger than 0.05 is enough to creter curvature effects. Curvature effects cn increase BL thickness using these different mechanisms: 1) Centrifugal forcing → Görtler vortices: creates streamwise counter-rotating vortices that redistribute momentum and produce localized thickening and heightened turbulence 2 )Pressure-gradient coupling: curvature commonly coexists with pressure gradients (adverse/favorable) which further modulate growth. 3 )Spanwise inhomogeneity: concave cases are often not spanwise uniform — so a single delta BL thicknes may hide large local variation (e.g., maxima vs minima related to vortex cores)



% -SoMellor (1975) show boundary layer on a concave wall becomes strongly three-dimensional and spatially inhomogeneous because concave curvature triggers a stationary system of longitudinal (Taylor–Görtler–type) vortices superposed on an otherwise conventional
% further argue that curvature has little effect very near the wall (near-wall similarity only marginal and log-law region collapses early, around , but it enhances outer-layer transport
% concrete mechanism for near-wall intermittency/heterogeneity and elevated dissipation on a concave stationary wall: curvature-induced longitudinal rolls can thicken/energize the outer part of the wall region and make boundary statistics highly nonuniform in the transverse direction, which can readily bias “boundary” eps upward 











%  -Patel’s work is essentially a warning that streamline curvature can produce first-order changes in turbulent boundary layers, and that you should not interpret wall-region behavior using flat-wall intuition when the centrifugal pressure field is appreciable: he reviews evidence from curved channels showing that turbulence production/intensity can be amplified near the outer (concave) wall  which would naturally raise near-wall mixing, entrainment and therefore local dissipation 
%  when it is 1/30 - 1/10 the effects can be severe; 
%  for concave surfaces one must expect and account for Görtler–Taylor-type instability vortices, which can make the “boundary layer” thicker, more three-dimensional and more intermittent than a canonical wall BL—exactly

%  - Saric’s review frames Görtler vortices as a centrifugal instability of boundary-layer-type shear over a concave wall (Rayleigh circulation mechanism), whose hallmark is a steady, streamwise-oriented pair of counter-rotating rolls with a fixed spanwise wavelength that grows downstream and then nonlinearly distorts the mean profile. The key consequence for dissipation is that these rolls redistribute streamwise momentum normal to the wall: upwelling lifts low-momentum near-wall fluid into the layer (locally reducing wall shear), while downwelling pushes higher-momentum fluid toward the wall (locally increasing wall shear), producing strong spanwise modulation (“streaks”) of wall shear stress and hence a highly inhomogeneous, bursty near-wall dissipation field (the review emphasizes that this profile distortion becomes “mushroom-shaped” and can reach a regime where spanwise gradients are comparable to wall-normal gradients). Once the distortion is strong, the review argues the flow is primed for secondary instabilities: a Kelvin–Helmholtz–type (“sinuous”) mode, and a Rayleigh-type (“varicose”) mode; these mechanisms create intense shear layers and unsteadiness, i.e. exactly the kind of process that would drive heavy-tailed, non-lognormal 
% eps PDFs and concentrated dissipation near the wall.

% \bigskip
% \paragraph{THE NATURE OF DISSIPATION IN A TURBULENT FLOW AND IN THE BL}

% ON THE NATURE OF DISSIPATION IN A TURBULENT FLOW AND IN THE BL:

% - Jiménez (2013) emphasizing that the shear-dominated near-wall region plays a central role in the production and dissipation of turbulent kinetic energy, even though it occupies a vanishingly small fraction of the flow volume at high Reynolds number. 
% local energy dissipation rate in the buffer and logarithmic layers increases toward the wall approximately as $epsilon(y) ~ u_tau^3 / (kappa y)$,
% As a consequence, while the viscous and buffer layers become geometrically thinner with increasing Reynolds number, The paper further shows that although the smallest scales of turbulence, including vorticity and velocity gradients, tend toward local isotropy away from the immediate wall, 
% Temporal intermittency in the form of bursting events is identified as a fundamental feature of near-wall turbulence, contributing significantly to both momentum transfer and dissipation.
% spatial organization imposed by the wall and the mean shear leads to dissipation that is strongly inhomogeneous and increasingly concentrated in near-wall regions as Reynolds number increases.
% this review synthesizes DNS/experimental evidence that, in smooth-wall turbulence, a disproportionate share of production and dissipation is wall-proximate and becomes increasingly “log-layer dominated” as Reynolds number grows. The core asymptotic argument is that, above the buffer layer, local production/dissipation scale like, so the integrated dissipation 
%  grows only logarithmically - implying that although the buffer layer is geometrically thin, it remains dynamically important even at high Reynolds numbers -  in the formal infinite-Re limit, essentially all dissipation sits in the log layer). 
%  the wall region exhibits strong temporal intermittency (“bursting”) in which wall friction/near-wall gradients spike sharply; 
% the wall–bulk contrast can grow with Re (log-layer–type concentration and wall-attached momentum-transfer events intensify in relative importance as the scale separation grows), and (ii) why dissipation PDFs near the wall can show strong non-lognormal behavior (bursty, intermittently organized near-wall events and amplitude modulation naturally generate heavy tails and strong spatial patchiness). In your case, any added wall-attached shear-layer effects and concave-wall centrifugal organization (Görtler-like roll/streak modulation) would plausibly enhance exactly the sort of spatially intermittent, streaky patterns




% -Ostilla-Mónico et al. (2016) DNS of Taylor–Couette flow show that large-scale Taylor rolls persist deep into the turbulent regime and remain dynamically active, transporting angular momentum through Reynolds stresses and imprinting their signature well inside the boundary layers. These rolls are wall-attached structures whose influence is felt even at distances very close to the wall, leading to strong spatial inhomogeneity and axial dependence of turbulence statistics. The authors show that the bulk region is characterized by nearly constant angular momentum, while very steep gradients are confined to thin boundary layers near the cylinders, indicating that transport and dissipation are highly localized. A



% - (Cadot et al., 1997; Lathrop et al., 1992) In such
% an inertially-driven turbulent flow, the bulk dissipation
% is much stronger than the dissipation in boundary layers



% In the classical three-dimensional turbulence phenomenology, energy is injected at large scales by the forcing mechanism, transferred downscale at a constant rate $\epsilon$ following
% a self-similar cascade, and then dissipated into heat at the Kolmogorov length scale, where viscous
% effects become dominant. On most realistic
% situations, however, the turbulence is anisotropic and/or inhomogeneous and/or non-stationary. In
% such cases, there is not any necessary equivalence between global energy injection, global energy dissipation, and local energy dissipation. 

% -A detailed
% comparison between  local estimate and the global energy dissipation rate in a Taylor-Couette
% flow at various Reynolds numbers has recently been made by Tokgoz et al.
% 1 using tomographic PIV
% measurements. They observe the estimate
% of local energy dissipation based on the velocity gradients and on the viscosity $\epsilon_\nu$ becomes increasingly inaccurate and underestimates the global energy dissipation

% -Kuzzay, Faranda 2015 - PIV and DR measure of dissipation show  he same localized structures of energy dissipation near the walls at
% x = +/-0.6, 
% energy dissipation in the middle part of the cells. Regarding instantaneous maps, it is interesting to
% note that it is characterized by intense, localized events that can reach 10–20 times the maximum
% average local dissipation. 

% -Duan, Chen Srennivasan 2025 - K41 :  In the inertial range where the cascade is thought to be inviscid and selfsimilar, K41 predicts that the velocity structure functions are determined only by avg($\epsilon$) and follow power law scaling $S_p(r) ≡ ⟨(\delta_r u)^p⟩ \approx (⟨\epsilon⟩r)^{p/3}$. 
%  Underlying K41 is the constancy of mean energy dissipation. In the presence of intermittency for real turbulence, the scaling laws for structure functions differ from K41, require modifications (termed anomalous scaling) of the type $S_p(r) \approx r^{\psi_p}$ , with the exponents $\psi_p$ depending nonlinearly on p, and must be determined separately for each p. 

 
% -Duan2025 takeaway is that walls don’t just “add a boundary condition” — they fundamentally change what dissipation looks like and where it lives. Using channel-flow simulations across Reynolds numbers, the authors show that away from the wall (in the outer part of the flow) dissipation behaves much like “bulk” turbulence: its strongest bursts grow in a way that’s consistent with classic intermittency ideas from homogeneous turbulence. Right at the wall, however, dissipation behaves differently: it forms streaky, highly structured patterns, and the way its extreme events scale with Reynolds number is much more constrained (“bounded”) than in the bulk. The net implication is that, as Reynolds number becomes very large, the bulk contribution becomes small compared to the wall contribution, so the wall increasingly controls the overall dissipation landscape; the authors even argue this points to solid boundaries being central to generating the kinds of “singular” dissipation behavior people associate with Onsager-type ideas. the dissipation PDF near boundaries should not be expected to look lognormal because the wall introduces strong shear, spatial organization, and distinct low-activity/high-activity structure compared with the core of the flow
% -Duan2025 - DNS of chanel flow -dissipation at the wall forms a streaky structure in the
% streamwise direction , with fluctuations reaching more intense extrema. An important quantitative detail of the patterns is revealed by the probability density functions (PDFs) of
% $\epsilon_{uu}$ in Fig. 2. In particular, the well-collapsed left tails
% have a distinct slope of -0.5 on the wall and 0.5 on the
% center (inset). These trends indicate a divergent PDF
% for zero dissipation at the wall and a vanishing PDF
% for the center. Both slopes have recently been reported
% in HIT for dissipation defined with different derivative
% terms [13, 14]. The oppositely signed slopes for the wall
% and the centerplane reflect different dynamics (also indicated by Fig. 1): they show that the standard energy cascade and the intermittency characteristic of the centerplane are strongly shaped at the wall by the shear, clearly
% amplifying the low-dissipation events (possibly also highamplitude events). They also highlight the role of the
% wall in shaping dissipation dynamics, leading to different
% scaling behaviors with changing distance from the wall,
% as stated toward the end of the Introduction.
% -Dissipation exhibits fundamentally different behaviors on the wall. As shown in Fig. 3b,
% wall dissipation increases with $Re_\tau$ , a trend that is in excellent agreement with the bounded defect law given by
% the wall/bulk contrast should grow with Re, which is qualitatively aligned with your finding that boundary eps exceeds the volumetric mean by an amount that increases with Re,
%  -  absence of intermittency at the wall might mean that universal bifractality as in HIT [47]. However, close to the wall, the bifractality simplifies to a unifractal. - Thus, for finite order p, (1) implies a negative
% scaling, hence vanishingly small dissipation in the bulk
% compared to that on the wall, for very large Reynolds
% numbers. This means that away from the wall, the flow
% does not generate sufficiently strong singularities. However, the extreme nature of dissipative events on the wall
% (compared to those in the bulk of the channel) suggests
% that walls may generate the necessary strength of singularities. This brings us to the broader possibility that
% the Onsager-type singularities [48, 49] might be generated  near the wall


% - KATO works: in bounded domains, energy dissipation in the vanishing-viscosity limit can concentrate in an increasingly thin boundary layer (of thickness O($\nu$) in Kato’s condition) — so the fraction of total eps coming from the walls can grow or remain finite as $\nu$ approaches 0 (Re appraoches inifty ), producing anomalous dissipation concentrated at the boundary. showed that the inviscid limit (Navier–Stokes to Euler) holds if and only if the viscous dissipation integrated over an O($\nu$)-thick boundary strip goes to zero. Equivalently, if there remains O(1) dissipation in that O($\nu$) strip as $\nu$ goes to 0, the viscous dissipation does not vanish and anomalous dissipation is concentrated at the boundary. The vlidity of this depedns on how BL thickness scales with Re or nu. 
% The persistence of a finite mean dissipation at high Reynolds number—the so-called dissipative anomaly—can arise from two complementary mechanisms. In unbounded or homogeneous flows, anomalous dissipation is associated with singular inertial dynamics in the bulk (Onsager 1949; Duchon and Robert 2000). In bounded flows, however, a second route exists: as viscosity decreases, steep velocity gradients within an 
% O($\nu$) boundary layer can yield an O(1)contribution to the total dissipation, a scenario formalized by Kato’s criterion (1984). 
% observation that the boundary‐layer dissipation fraction grows with Re may represent the wall-dominated realization of the dissipative anomaly. The bulk inertial cascade maintains a nearly Re-independent mean eps, while increasingly concentrated wall gradients ensure that the total energy flux is absorbed within the near-wall region rather than uniformly in the volume.





% - Kato showed that (for sufficiently regular Euler solutions) Navier–Stokes solutions  converge to Euler if and only if the viscous dissipation associated with velocity gradients in an extremely thin boundary strip of thickness vanishes: 
% . Kelliher proves this is equivalent to requiring the same vanishing criterion using vorticity instead of 
%  and (with extra regularity) also equivalent to a condition on kinetic energy in the strip:. In other words, whether the inviscid limit holds is controlled entirely by what happens in a vanishingly thin near-wall region; if that region retains finite dissipation/vorticity activity, it can block convergence even if the bulk looks “Euler-like.
%  the Kato/Kelliher viewpoint suggests a sharp interpretation: you may be approaching a regime where the bulk increasingly behaves like an inviscid (Euler/Onsager-type) flow, while the net energy loss is progressively localized to the boundary, ie  an emerging boundary-controlled dissipation anomaly.
% A direct experimental diagnostic in your framework is to estimate (or bound) the fraction of total dissipation contained in a strip whose thickness scales like nu - precisely the scenario Kato identifies as the inviscid-limit failure mode

% -Drivas & Nguyen extend Onsager-style energy conservation/dissipation criteria to bounded domains by cleanly separating bulk versus near-wall mechanisms: they prove that a weak Euler solution conserves energy if (i) in every interior subdomain the velocity has Onsager-critical Besov regularity  and (ii) in an arbitrarily thin neighborhood of the wall the fields are bounded and the wall-normal velocity is continuous; they then establish analogous inviscid-limit theorems for Leray–Hopf Navier–Stokes solutions showing that global viscous dissipation must vanish as 
% nu →0 if those bulk-regularity and near-wall boundedness/continuity assumptions hold uniformly in a boundary strip whose thickness can shrink with 
% nu (a “Kato-type” layer, with a width scaling like ). Their discussion is directly relevant to your “wall dissipation rises while bulk stays flat/decreases” observation because it gives a sharp interpretation: if your bulk increasingly behaves “Euler-like” (i.e. consistent with improved interior regularity / reduced bulk anomaly) but the wall contribution remains strong, then the only way to retain nontrivial dissipation in the high-Re (small- nu) limit is via boundary-driven mechanisms—either (a) a failure of the near-wall boundedness/continuity assumptions, or (b) non-vanishing dissipation inside a vanishingly thin wall strip (the Kato-layer failure mode), which is precisely the setting where “singular” objects such as vortex sheets shed from the wall can sustain dissipation even when the interior does not. 




% -Benzi et al. (1999) show—using long-time DNS of turbulent channel flow—that intermittency of velocity increments strengthens markedly as you approach the wall, even though scaling laws persist there, and they trace this to a breakdown of the usual refined Kolmogorov similarity hypothesis (RKSH) in the near-wall region: 
%  They propose a new wall-region RKSH in which the relevant “flux-like” quantity becomes the second-order structure function—physically because in strong shear a term proportional to ? enters the scale-by-scale energy transfer and can dominate the usual inertial transfer  A key point for your von Kármán wall dissipation results is their conclusion that the observed rise of intermittency near the wall is not primarily explained by stronger intermittency of the dissipation field itself (they find the inferred intermittency correction from dissipation statistics is essentially independent of wall distance), but rather by a change in the governing transfer mechanism: near-wall dynamics are “controlled more by momentum transfer toward the wall than by the classical energy cascade.”
 

% -Hartel, Kleiser, Unger and Friedrich (1994) use DNS of turbulent channel and pipe flow 
% while the mean SGS dissipation (net transfer from resolved to subgrid) is non-negative overall, the fluctuation-driven component becomes negative around y+ = 12, indicating a mean backscatter / reverse transfer (small to large scales) localized to the buffer layer; this reverse transfer is attributed primarily to SGS stresses aligned with the mean strain and cannot be captured by purely dissipative eddy-viscosity closures. Using stress–strain correlations and conditional averaging, they show that strong negative-transfer events are strongly enhanced by coherent near-wall motions (“bursting”) and appear as extended attached high-shear layers reaching from the wall up toward the edge of the buffer layer (order 
% y+ =40), i.e. the energetics in the wall region are organized by intermittent coherent structures rather than a simple monotone forward cascade. 


% -Hack and Schmidt 2019 analyze extreme dissipation events in time-resolved DNS of a turbulent boundary layer by identifying local maxima of the dissipation of turbulent kinetic energy  at fixed wall distances 
% y+= =20,30,60,150), and show that these peaks are highly intermittent: vast regions of weak activity are punctuated by rare spikes whose intensity increases strongly as the wall is approached (their event-intensity histograms at each 
%  are “remarkably well described” by log-normal fits, but only a tiny fraction 
% 0.4 - 0.9 perce of maxima exceed the thresholds used for conditioning) (pp. 3–5). The key physical finding is that conditioning on dissipation peaks consistently extracts the same coherent mechanism across the buffer and into the outer layer: a strong ejection/burst (positive  associated with a low-speed streak beneath a high-speed patch, consistent with varicose streak instability, and accompanied by hairpin-like structures in ; importantly, the conditional fields show that peak dissipation coincides with peak production and peak 
%  (with production peaking slightly closer to the wall), and the time evolution of peak quantities exhibits approximately exponential growth/decay with a characteristic timescale that varies with wall distance (pp. 6–9). 
%  if your wall dissipation is dominated by rare, spatially localized “events,” then (i) your non-lognormal PDFs and Re-growing wall/bulk contrast can naturally arise from changes in event rate, amplitude, or footprint, and (ii) a very clean next step is to replicate their event-conditioned averaging using your wall-
% eps  maxima to see whether your strongest wall events also align with a repeatable instability/burst mechanism (in your case potentially fed by curvature/Görtler modulation or wall-attached shear-layer attachment), and to quantify how much of 
% eps avg is carried by the top 
% 0.1-1 percent  of events.




% -Buono et al. (2024) compile DNS, lab (TBL/open-channel/pipe) and atmospheric data to show that in smooth-wall turbulent flows  the “up-and-down” motion of the fluid in the region a little away from the wall has a surprisingly consistent bias: upward motions are slightly stronger or more frequent than downward motions, and this bias looks very similar across flows and Reynolds numbers once you are in that intermediate region between the viscous near-wall zone and the outer flow. In other words, there’s a kind of universal asymmetry in how fluid moves away from and toward the wall.


% -Meneveau & Sreenivasan (1991) show that turbulent energy dissipation is best viewed as a multifractal (multi-scaling) field generated by an underlying multiplicative cascade, rather than something that can be captured by a single “intermittency parameter” or a lognormal model. 
% supporting the idea of fairly universal inertial-range intermittency.
% demonstrate that the tails of coarse-grained dissipation distributions decay faster than lognormal, and are better described by a stretched (square-root) exponential tail form; 
% your data are unusually well-suited to test this cleanly by computing multifractal spectra / generalized-dimension curves separately for wall and bulk, checking whether the wall has a systematically different spectrum (signaling genuinely different small-scale organization/energy transfer in the wall-attached shear region) rather than just a mean-level shift.



% -KArtik 2025 - This PRL argues that the classic “zeroth law” idea—namely that the average rate at which turbulence dissipates energy stays essentially constant as viscosity becomes very small—may not be as universal as often assumed when the flow has no solid boundaries. Using a sequence of high-resolution simulations of homogeneous, wall-free turbulence in a periodic box, the authors find evidence that the mean dissipation likely decreases slowly as Reynolds number increases, rather than approaching a strict nonzero constant; 
% they interpret this as suggesting that turbulence without walls may not generate strong enough extreme gradients to sustain the strongest form of the dissipation anomaly. 


% -CLAIM: walls fundamentally reorganize dissipation statistics: can we show less intermittency at the wall as compared to flow center

% does this inform the multi-fractal view of turbulence ? 

